Agent Error Dataset: Scaling 50,000 Error--Diagnosis Pairs for Failure Analysis and Error-Aware Post-Training

An unsuccessful LLM agent rollout contains more information than its final reward: the observations available to the agent, the actions it chose, and the environment's responses. Reusing this experience for learning requires identifying a decision to revise and testing a concrete alternative. We introduce the Agent Error Dataset (AED), comprising 50,228 error-diagnosis pairs from 9,961 source tasks across 33 environments, 19 harness families, and 23 policy models in text-based agent systems. We retain source traces and execution metadata to support cross-setting failure analysis and re-diagnosis without repeating the original rollout. Our five-stage Agentic Error-to-Training (AET) pipeline collects natural failures, generates diagnoses and proposed corrections, and checks them against recorded evidence. Where replay is supported, we compare corrections with original-action retries from the same checkpoint under matched execution settings. We then construct separate training views for diagnosis and actor recovery. Across 3,062 matched replay pairs, first-proposal corrections raise verifier pass rates from 18.4% to 51.1%, a gain of 32.7 percentage points. Using a separately frozen diagnosis release, full-diagnosis fine-tuning on 1,656 source tasks raises Qwen3-8B's exact-step agreement with internal teacher labels from 47.2% to 63.6%, averaged over three seeds on a 943-case holdout. The strongest prompted reference in this comparison scores 54.7%, and mean agreement improves at each of four increasing training-set sizes. In a single-seed comparison of actor-training recipes, action-only repair training scores 6.67 percentage points higher on WebShop-lite than success-only training.

==> title_branding.tex <==
% Visual styling only. The main-file title wording and empirical claims are unchanged.
% Mark cropped from the existing Sunburst artwork, not a new image-model invocation.
% Provenance: reports/paper_visual_polish_20260923/title_mark.json.
\RequirePackage{etoolbox}
\definecolor{aedtitleblue}{HTML}{087FA6}
\definecolor{aedtitleindigo}{HTML}{315BD7}
\definecolor{aedtitlepurple}{HTML}{7C3DB4}
\newcommand{\aedtitlemark}{\raisebox{-.17em}[0pt][0pt]{%
  \includegraphics[height=1.15em]{figures/aed_title_mark_20260923.png}}\hspace{.25em}}
\makeatletter
\AtBeginDocument{%
  \patchcmd{\@title}{Agent Error Dataset:}%
    {\aedtitlemark\textcolor{aedtitleblue}{Agent}~\textcolor{aedtitleindigo}{Error}~\textcolor{aedtitlepurple}{Dataset}:}%
    {}{\PackageError{aed-title}{Expected title prefix not found}{Review title branding after the main title changes.}}%
}
\makeatother

